Generative Interventions for Causal Learning

We introduce a framework for learning robust visual representations that generalize to new viewpoints, backgrounds, and scene contexts. Discriminative models often learn naturally occurring spurious correlations, which cause them to fail on images outside of the training distribution. In this paper, we show that we can steer generative models to manufacture interventions on features caused by confounding factors. Experiments, visualizations, and theoretical results show this method learns robust representations more consistent with the underlying causal relationships. Our approach improves performance on multiple datasets demanding out-of-distribution generalization, and we demonstrate state-of-the-art performance generalizing from ImageNet to ObjectNet dataset.

==> source/backup.tex <==
\begin{table*}[t]
\begin{center}
    \centering
    \begin{tabular}{ll|cc|cc}
         \toprule
         & & \multicolumn{2}{c|}{Std.\ Augmentation}  & \multicolumn{2}{c}{Add.\ Augmentation}\\
         Backbone & Training Distribution & top1   & top5  & top1 & top5\\
         \midrule  
        % \parbox[t]{1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ResNet18}}}
         \multirow{3}{*}{ResNet18 \cite{He_2016}} & ImageNet Only \cite{He_2016}  & 20.48\% & 40.64\% & 24.42\% & 44.39\% \\
         &Stylized ImageNet \cite{imagenetbiased} & 18.39\% & 37.29\% & 22.81\% & 42.27\% \\
         &Mixup \cite{zhang2017mixup} & 19.12\% & 37.78\% & cv04 \\
         &AutoAug \cite{cubuk2018autoaugment} & 21.20\% & 41.26\% & 21.20\% & 41.26\% \\
         & Observational GAN \cite{CAS}  & 20.63\%  & 39.77\% &  23.72\% & 43.67\% \\
         & Interventional GAN (ours)  & 22.07\% & \textbf{41.94\%} &  25.71\% & 46.39\%\\
         & Intervention GAN Transfer (ours) & 22.29\% & 41.76\% & 27.02\% & 47.51\% \\
         & Interventional GAN Combined (ours) & \textbf{22.34\%} & 41.65\% & \textbf{27.03\%} & \textbf{48.02\%} \\
         
         \midrule  
        %  \parbox[t]{1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ResNet152}}}
          \multirow{5}{*}{ResNet152 \cite{He_2016}} & ImageNet Only  \cite{Objectnet} & 30.00\% & 48.00\% & - & -\\
          & ImageNet Only$\dagger$ w/o crop & 31.01\% & 52.46\% & 33.03\% & 53.75\% \\
          & ImageNet Only$\dagger$ w/ crop & 34.19\% & 55.58\% & 37.43\% & 59.10\% \\    % this is best: tune additional 20 epoch\\
          & Stylized ImageNet \cite{imagenetbiased} & 31.64\% & 52.56\% &  \\
          & Mixup \cite{zhang2017mixup} & 34.27\% & 55.68\% \\
          & AutoAug \cite{cubuk2018autoaugment} & 33.96\% & 55.81\% & 33.96\% & 55.81\% \\
          & Observational GAN \cite{CAS} & 33.17\% & 54.59\% & 36.37\% & 58.88\%\\
          & Interventional GAN (ours) & \textbf{35.12\%} & \textbf{56.94\%} & 39.21\% & 61.06\% \\ % only tune 10 epoch \\
          & Interventional GAN transfer (ours) & & & \textbf{39.44\%} & \textbf{61.56\%} \\
         
         \bottomrule
    \end{tabular}
\end{center}
\caption{Accuracy on the ObjectNet test set versus training distributions. The $\dagger$ indicates that we-reimplemented the baseline, which performed better than the published baseline. By intervening on the training distribution with generative models, we obtain state-of-the-art performance on the ObjectNet test set, even though the model was never trained on ObjectNet.} \label{tab:objectnet}
\end{table*}






\begin{table}[t]
    \begin{tabular}{l|cc|}
         \toprule
         Training Distribution & top1   & top5  \\
         \midrule  
        %  \parbox[t]{1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ResNet152}}}
          %ImageNet Only w/o crop & 76.26\% & 93.34\%  \\
          ImageNet Only \cite{He_2016} & 78.57\% & 94.29\% \\    % this is best: tune additional 20 epoch\\
           Observational GAN  & 79.16\% & 94.63\% \\
           Interventional GAN (ours) & 79.15\% & 94.55\% \\ % only tune 10 epoch \\
         \bottomrule
    \end{tabular}
\caption{Accuracy on ImageNet validation set. Our approach also improves performance on ImageNet, suggesting the model generalizes to new datasets without sacrificing the performance on the original dataset.}
\label{tab:imagenet}
\end{table}



\begin{table*}[t]
\centering
\setlength{\tabcolsep}{4pt}
\scriptsize
    \begin{tabular}{l|c|ccc|cccc|cccc|cccc}
         \toprule
         Model & \textbf{mCE $\big\downarrow$} & Gauss. & Shot & Impulse & Defocus & Glass & Motion & Zoom & Snow & Frost & Fog & Bright & Contrast & Elastic & Pixel & JPEG \\
         \midrule  
          AlexNet & 100.00 &100 &100 &100 &100 &100 &100 &100 &100 &100 &100 & 100 &100 &100 &100 &100  \\
          \midrule
          ImgNet Only \cite{He_2016} & 87.16 & 89.5&	90.4&	93.0 &	86.01 &	93.3 &	87.7 &	90.0 &	87.5 &	86.4 &	80.0 &	73.7 &	80.5 &	91.5 &	85.5 &	92.4 \\    % this is best: tune additional 20 epoch\\
          Stylized ImgNet \cite{imagenetbiased} & 80.83 & 79.1&	80.9&	81.7&	81.7&	87.6&	80.0&	90.0&	78.3&	80.2&	76.2&	72.5&	77.2&	84.1&	76.2&	86.7\\
          Mixup \cite{zhang2017mixup} & 86.06 & 86.8 &	88.1&	90.8&	88.7&	95.6&	89.1&	89.3&	82.5&	72.8&	71.9&	75.9&	76.5&	96.2&	89.5&	97.2\\
          Autoaug \cite{cubuk2018autoaugment}  & 84.00 & 84.3&	83.7&	84.5&	87.9&	93.6&	87.7 &	93.5&	85.7&	83.4&	71.0&	67.4&	63.5&	97.8&	85.3&	90.5 \\
          Observational GAN \cite{CAS} & 86.48 & 86.4&	87.5&	90.5&	87.0&	92.4&	87.2&	90.3&	88.0&	86.3&	82.8&	73.3&	82.8&	90.7&	84.5&	87.5 \\
           Interventional GAN (ours) & \textbf{74.68} & 67.0&	68.4&	67.3&	75.0&	80.5&	76.0&	84.2&	77.4&	75.9&	77.5&	68.8&	76.6&	87.5&	59.8&	77.5  \\ % this is combined int gan
         \bottomrule
    \end{tabular}
\caption{Corruption on the nuisances should not cause the label. We show mean corruption error (mCE $\downarrow$) rate (the smaller the better) on ImageNet-C validation \cite{imgnet-C} set with 15 different corruptions. We normalize CE with AlexNet \cite{imgnet-C}. Our intervention GAN, without training on any of the corruptions, reduces the mCE by up to \textbf{12.48\%} on ResNet 18 model. We show individual gain on each corruptions. Without explicitly adding similar corruption in the training, our generative intervention strategy naturally learns more causal features instead of the nuisances bias.} %All models are trained with the same number of iterations. 
\label{tab:imagenet-C}
\end{table*}
% For example, on the ``zoom'' task, while all the baseline methods are not able to reduce the error from the baseline, we reduce it by 5.8\%, since our interventional GAN removes the zoom confounding bias (See Component 10 in Figure \ref{fig:equi}).







% Table results for Imagenet and ImageNet-v2 on Res152 and Res18


\begin{table*}[t]

    \begin{tabular}{l|cc|cc|cc||cc}
         \toprule
         
         & \multicolumn{2}{c|}{Top Score} & \multicolumn{2}{c|}{Thre 0.7} & \multicolumn{2}{c||}{Matched Freq} & \multicolumn{2}{c}{ImageNet Val}  \\
         Training Distribution & top1   & top5 & top1   & top5 & top1   & top5  & top1   & top5 \\
         \midrule  
        %  \parbox[t]{1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ResNet152}}}
          %ImageNet Only w/o crop & 76.26\% & 93.34\%  \\
          ImageNet Only \cite{He_2016} & 71.77\% & 91.11\% & 65.41\% & 87.39\% & 56.18\% & 79.35\% & 68.82\% & 88.96\%\\    
          Stylized ImageNet \cite{imagenetbiased} & 69.55\% & 89.97\% & 62.92\% & 85.38\% & 54.13\% & 77.30\% & 66.95\% & 87.42\%\\
          Mixup \cite{zhang2017mixup} & 69.90\% & 90.16\% & 63.42\% & 86.40\% & 54.42\% & 77.94\% & 66.00\% & 86.93\%\\
          AutoAug \cite{cubuk2018autoaugment} & 72.05\% & 91.49\% & 65.32\% & 87.32\% & 56.25\% & 79.16\% & 69.24\% & 88.91\%\\
          
           Observational GAN \cite{CAS}  & 72.01\% & 91.24\% & 65.72\% & 87.58\% & 56.43\% & 79.42\% & 69.19\% & 88.85\% \\
           \midrule
           Interventional GAN & 72.80\% & \textbf{91.89\%} & 66.26\% & 88.30\% & \textbf{57.86\%} & \textbf{80.11\%} & \textbf{70.41\%} & 8\textbf{9.59\%} \\
           Interventional GAN Transfer  & \textbf{72.96\%} & 91.84\% & 65.93\% & \textbf{88.31\%} & 57.42\% & 79.84\% & 70.13\% & 89.38\% \\
           
           Interventional GAN Combined & 72.84\% & 91.85\% & \textbf{66.49\%} & 88.11\% & 57.35\% & 79.61\% & 70.25\% & 89.33\%\\
           
           % only tune 10 epoch \\
         \bottomrule
    \end{tabular}
\caption{Accuracy on ImageNet V2 validation set \cite{ImageNetOverfit}. Our approach also improves performance on ImageNet-V2, suggesting the model generalizes to new validation datasets.}
\label{tab:imagenet-v2-18}
\end{table*}



\begin{table*}[t]
    \begin{tabular}{l|cc|cc|cc||cc}
         \toprule
         
         & \multicolumn{2}{c|}{Top Score} & \multicolumn{2}{c|}{Thre 0.7} & \multicolumn{2}{c||}{Matched Freq} & \multicolumn{2}{c}{ImageNet Val}  \\
         Training Distribution & top1   & top5 & top1   & top5 & top1   & top5  & top1   & top5 \\
         \midrule  
        %  \parbox[t]{1mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{ResNet152}}}
          %ImageNet Only w/o crop & 76.26\% & 93.34\%  \\
          ImageNet Only \cite{He_2016} & 81.01\% & 96.21\% & 76.17\% & 94.12\% & 67.76\% & 87.57\% & 78.57\% & 94.29\% \\    
          Stylized ImageNet \cite{imagenetbiased} & 79.40\% & 95.72\% & 74.02\% & 92.88\% & 65.12\% & 86.22\% & 77.27\% & 93.76\% \\
          Mixup \cite{zhang2017mixup} & 80.68\% & 96.28\% & 75.91\% & 94.00\% & 67.11\% & 87.66\% & 78.78\% & 94.45\% \\
          AutoAug \cite{cubuk2018autoaugment} & 80.61\% & 96.30\% & 75.90\% & 94.06\% & 67.35\% & 87.61\% & 78.95\% & 94.56\%\\
          
           Observational GAN \cite{CAS}  & 80.10\% & 96.00\% & 75.60\% & 93.74\% & 66.89\% & 87.04\% & 78.53\% & 94.21\% \\
           \midrule
           Interventional GAN & 80.77\% & \textbf{96.38\%} & 76.20\% & \textbf{94.24\%} & 67.74\% & \textbf{87.83\%} & 79.46\% & 94.71\% \\
           Interventional GAN Transfer  & 81.04\% & 96.15\% & 76.13\% & 93.89\% & 68.08\% & 87.83\% &79.51\% & 94.81\% \\
           
           Interventional GAN Combined & 
            \textbf{81.24\%} & 96.28\% & \textbf{76.60\%} & 93.95\% & \textbf{68.08\%} & 87.70\%& \textbf{79.59\%} & \textbf{94.79\%} \\
           
           % only tune 10 epoch \\
         \bottomrule
    \end{tabular}
\caption{Resnet152 accuracy on ImageNet V2 validation set \cite{ImageNetOverfit}. Our approach also improves performance on ImageNet-V2, suggesting the model generalizes to new validation datasets.}
\label{tab:imagenet}
\end{table*}








\subsection{Causal Effect Bound}
Imperfect interventions can eliminate only some spurious correlations. Though it is theoretically impossible to calculate the exact causal effect $P(y|do(x))$ when spurious correlations are not totally removed, we can still estimate the lower and upper bound for $P(y|do(x))$.

 Given the observed joint distribution $P(x,y)$, Pearl \cite{pearl} identified that $P(y|do(x))$ can be bounded by $P(x,y) \le P(y|do(x)) \le P(x,y)+1-P(x)$, which can be estimated by existing discriminative models without interventions. 
 
 Prior work augments the data by sampling from the GANs without explicit intervention~\cite{lowshotgan, antoniou2017gandataaug, GANaug, GanLiver}, which will yield the same causal bound as the original data. Since GANs capture the same distribution as the observational training set, the spurious correlations remain the same. The sampled transformations $Z$ in Figure \ref{fig:causalgraph} (a) are still dependent on the confounders $C$. Thus, augmenting training data with GANs \cite{CAS}, without intervention is not an effective algorithm for causal identification. 

In this paper, we aim to identify a tighter causal effect bound for $P(y|do(x))$ using generative interventions. This is desirable for robustness because it removes or reduces the overlap between the causal intervals, promoting causal predictions. 
Section~\ref{sec:dis} establishes that perfect interventions eliminate all spurious correlation and leads to better generalization. In practice, our generative interventions may only eliminate a subset of spurious correlations  $Z_i$, while other nuisances $Z_U$ remain unobserved and untouched. The next question is then: \emph{what generative intervention strategy is optimal for tightening the causal effect bound?} We derive the following theory:


% \textbf{Eliminating spurious correlation helps generalization.} 

% As shown in , our intervention on nuisances $Z_i$ removes the spurious correlations from $Z_i$ to label $Y$, which shifts the distribution of the generated images $X$ independently of the some of the confounding factors $C$.




% The proper intervention needs to 
%  Our derived theorem can also explain a boarder range of partial intervention strategies.

\begin{theorem}[\textbf{Effective Intervention Strategy}]\label{th:2IV}
We denote the images as $x$. The causal bound under intervention $z_i$ is thus $P(y,x|z_i) \leq P(y|do(x)) \leq P(y,x|z_i) + 1 - P(x|z_i)$. For two intervention strategies $z_1$ and $z_2$,  $z_1 \subset z, z_2 \subset z$, if  $P(x|z_1) > P(x|z_2)$, then $z_1$ is more effective for causal identification. 
\end{theorem}

\begin{proof}
% We denote all the unobserved confounding variables as $u$.
Figure \ref{fig:causalgraph}(c) shows the causal graph after intervention $Z_i$, where $Z_i \independent Y | X$.  We add and remove the same term $\sum_c P(y,x,c|z_i)$:
% \begin{align*}
% P(y|do(x)) &= P(y|do(x), do(z)) = P(y|do(x), z) = \sum_c P(y|x,z,c)P(c)\\   % \sum_u P(y,x,u|z)
% &= \sum_c P(y,x,c|z) + \sum_c{P(y|x,z,c)(P(c)-P(x,c|z))}
% \end{align*}
\begin{align*}
\begin{split}
& P(y|do(x)) = \sum_c P(y|x,z_i,c)P(c) \quad  \text{(Backdoor Criteria)} \\
&= \sum_c P(y,x,c|z_i) + \sum_c{P(y|x,z_i,c)(P(c)-P(x,c|z_i))}
\end{split}
\end{align*}
Since $0 \leq P(y|x,z_i,c) \leq 1$, we have the lower and upper bounds. 
We denote $\delta_1 = P(x|z_1) - P(x|z_2)$, thus  $\delta_1>0$. In the causal graph (Figure \ref{fig:causalgraph}(c)), since we intervene on $z_i$, all incoming edges  to $z_i$ are removed; 
we then have $z_i \independent y | x$ and $P(x,y|z_i) = P(y|x,z_i)P(x|z_i)= P(y|x)P(x|z_i)$. Therefore $\delta_2=P(x,y|z_1)-P(x,y|z_2)=\delta_1 \cdot P(y|x)$. %, then $\delta_2 = \delta_1 \cdot P(y|x)$. 
Since $0<P(y|x)<1$, we have $0<\delta_2<\delta_1$. Thus we obtain $[P(y,x|z_1), P(y,x|z_1) + 1 - P(x|z_1)] \subset [P(y,x|z_2), P(y,x|z_2) + 1 - P(x|z_2)]$, which means the intervention $z_1$ results in a tighter causal effect bound.
% \begin{align*}
% P(y|do(x)) &\leq \sum_c P(y,x,c|z) + \sum_c(P(c)-P(x,c|z)) = P(y,x|z) + 1 - P(x|z)\\
% P(y|do(x)) &\geq \sum_c P(y,x,c|z) = P(y,x|z)
% \end{align*}
% \begin{align*}
% P(y,x|z_i) \leq P(y|do(x)) \leq P(y,x|z_i) + 1 - P(x|z_i)
% \end{align*}
% For the chosen interventional variable $z_1$ and $z_2$, the identifiable bound is $I_1 = [P(y,x|z_1), P(y,x|z_1) + 1 - P(x|z_1)]$ and $I_2 = [P(y,x|z_2), P(y,x|z_2) + 1 - P(x|z_2)]$.
\end{proof}
% 
% Given the conditions $P(x,y|z_1) = P(x,y|z_2) + \delta_2$,  $\delta_1 > \delta_2 > 0$,
% , then $L_1<L_2$, which means the  length of the bound interval is smaller. 
% , and the interval length is $L_1=1 - P(x|z_1)$ and $L_2=1 - P(x|z_2)$ respectively

Our theorem shows that: the optimal intervention strategy should maximize $P(x|z)$, which will tighten the causal effect bound $P(y|do(x))$. In addition, the intervention strategy should be identically selected across all categories, so that they are independent of the confounding bias. While there are different choices of intervening on the generative model to create independence, we empirically select our generative intervention strategy that increases $P(x|z)$, which we will discuss in Section \ref{sec:int_effect}.


==> source/method_old.tex <==


\section{Method}
\label{sec:method}
 We show how deep generative models can be used to construct interventions on the spuriously correlated features in the causal graph. We combine these results to develop a practical framework for robust learning. 


\subsection{Learning}

\subsection{Generative Interventions}

Conditional generative adversarial networks (CGAN) are a class of generative models that learn the mapping $x = G(\h_0,\y)$ where $\h_0 \sim \mathcal{N}(0, I)$ is a latent vector, $\y$ is a class label, and $\x$ is a generated image of class $\y$ that lies in the natural image distribution. CGANs are trained on the joint data distribution $P(x,y)$. While we can use any type of conditional generative models, we use the BigGAN model \cite{BigGAN} in this paper. In addition to producing highly realistic images, generative models learn a latent representation $\h_0$ that is steerable \cite{hrknen2020ganspace, jahanian2019steerability}, allowing for controlled visual manipulation.
%Since the model is conditional, a random walk along $h$ will generate images that are still representative of the class $y$.
For example, \cite{hrknen2020ganspace} empirically showed that the principal components of $\h$ correspond to visual transformations over camera extrinsics and scene properties. The same perturbations in the latent space will produce the same visual transformation across different categories. Figure \ref{fig:equi} visualizes this steerability for a few samples and different transformations. 
This property enables us to construct a new training distribution, where the nuisances features $Z$ are not affected by the confounders (Figure \ref{fig:spurious_measure}). 

% The theorem suggests that we should select the interventions that maximize $P(X|Z)$.

We define the transformations to be along the principal directions $\r$ in the feature space \cite{hrknen2020ganspace}, which are orthogonal and capture the major variations of the data. We select the top-k significant ones as the intervention directions. We then intervene along the selected directions with a uniformly sampled step size from a range. We intervene on the generator's intermediate layers with $\h_i^* = \h_i + \sigma s \r - \mu $, where $\h_i$ are the features at layer $i$, $s$ is the scaling factor, $\sigma$ is the standard deviation of noise on direction $\r$, and $\mu$ is the offset term. After the intervention, we recover $\h_0^*$ with linear regression \cite{hrknen2020ganspace} and generate the new image $\x^* = G(\h_0^*, \y)$.
 Using conditional generative models, we produce the causal features $X_F$ by specifying the category. Our intervention on $Z$ removes the incoming edge to $Z$ (Figure \ref{fig:causalgraph} (b)). We empirically choose the hyper-parameters $k, s$ that increases $P(x|z)$ the most (Figure \ref{fig:intervention}). In practice, there are some transformations $Z_U$ that the generator will fail to capture (Figure \ref{fig:causalgraph} (c)). Though the missing factors would remain as back-doors for the causal effect identification, our theory shows that the intervention still tightens the causal effect bound.
 
\subsection{Leveraging Existing Data}

% (\cv{Key point: It's actually acceptable if a transformation causes two different changes (eg viewpoint and color). We only care that z is changed, not f.}
%  a principal direction may cause multiple alterations (e.g.\ viewpoint and color), but due to our uniformly sampled intervention strategy, $Z$ will be independent to the confounding factors $C,E$ regardless.  Nevertheless, 

%Note that our theory, which we present next, still applies even when we cannot intervene on some confounding factors. 

%  Due to the architecture design of generative model \cite{BigGAN, kingma2013autoencoding}, the resulting causal graph is Figure 1b, where transformation $z$ is constructed by given target (bidirected arrow) and random noise (unobserved variables not plotted). 


% \subsection{Generating Interventions} \label{subsec:algorithm}

% The above sections shows interventions on the generative models can shift the training distribution to be independent of the spurious factors in the original training data. 

 

% We describe our intervention details in the followings.          

% Our theory suggests that we are able to learn more robust representations by  using interventions.   We propose the following approach for learning:

% \textbf{Conditional Generation:} 
% Conditional generative models are trained on the full training data $P(x|y)$. Conditioned on a class label, samples from the trained generative model will produce images from the provided class. We denote the latent vector as $\h_0 \sim \mathcal{N}(0, I)$, the assigned label as $\y$, and the deep generative neural network as $G(\h_0, \y)$. The image $\x$ is generated by a forward pass of the generator $\x = G(\h_0, \y)$. While we can use any type of conditional generative model, we use  the bigGAN model \cite{BigGAN}.

% either variational auto-encoders \cite{kingma2013autoencoding} and

%\textbf{Steering the Generator:}


% To create variations efficiently in the high dimensional latent space, we calculate the principal components \cite{hrknen2020ganspace} and .

% We sample those directions with equal possibility to remove the data bias on transformations. 

% randomize the variation uniformly in an anisotropy feature space,  with equal possibility.
% As shown in Figure \ref{fig:equi}, these transformations are independent to the category, thus such interventions 

% Let $\r$ be the direction of a principal component for the features at a layer $i$ in the generator. 
% Since our intervention only changes the latent noise $\h_0$, while the assigned label $\y$ is the same, the generated data $\x^*$ maintains the causal features $F$ for the object class. 

% that shifts the random initial point to the mean value
% value randomly sampled from the intervention scale $[-I, I]$



%Visualization of interventions in Figure \ref{fig:equi}.

% Taking advantage of the emerging confounding factors of deep generative models, we generate new data by steering the generator with controlled intervention.
% Assume the direction for steering a certain confounding factor to be $\c$, following the method in \cite{hrknen2020ganspace}, 

\subsection{Training on Interventional Data}

The new intervened data can be used to learn more robust causal representations.
We train the full model with the generated data and the original data. We denote the original data matrix as $\X$ and the target labels as $\Y$, the generated data matrix as $\X'$ and the target labels as $\Y'$, and the discriminative classifier as $\phi$. 

Note that the original data will add the confounding bias back to our model. While our theory shows our method can still tighten the causal effect bound under the presence of spurious correlations, it is desired to also intervene on the original data. One straight approach to do this is to find the latent code in the generator that can generate the queried image, then apply our aforementioned algorithm for intervention. However, projecting the images back to the latent space in the generative models still remains as an open challenge \cite{zhu2018generative, huh2020ganprojection}. Instead, we propose to transfer the desired intervention from $X'$ to the original data $X$ with neural style transfer \cite{style_transfer}. The category information is maintained by the matching loss while the intervened nuisance factors is transferred via minimizing the maximum mean discrepancy \cite{li2017demystifying}. While the transfer is not ideal, we can still intervene on some of the nuisance factors $z$ in the original data, such as the background. We denote these data as $\X''$ and their corresponding label as $Y''$. We minimize the following training loss on our intervened data:
\[ \mathcal{L} = \lambda_1 \mathcal{L}_{e}(\phi(\X),\Y) + \lambda_2 \mathcal{L}_{e}(\phi(\X'),\Y') + \lambda_3 \mathcal{L}_{e}(\phi(\X''),\Y'') \]
where $\mathcal{L}_{e}$ denotes the standard cross entropy loss and $\lambda_1, \lambda_2,\lambda_2 \in \mathbb{R}$ are hyper-parameters controlling different training data choice. 


==> source/removed.tex <==


